The First Tidally Disrupted Ultra-Faint Dwarf Galaxy? - Spectroscopic Analysis of the Tucana III Stream

We present a spectroscopic study of the tidal tails and core of the Milky Way satellite Tucana III, collectively referred to as the Tucana III stream, using the 2dF+AAOmega spectrograph on the Anglo-Australian Telescope and the IMACS spectrograph on the Magellan/Baade Telescope. In addition to recovering the brightest 9 previously known member stars in the Tucana III core, we identify 22 members in the tidal tails. We observe strong evidence for a velocity gradient of 8.0 km/s/deg (or 18.3 km/s/kpc over at least 3$^{\circ}$ (or 1.3 kpc) on the sky. Based on the continuity in velocity we confirm that the Tucana III tails are real tidal extensions of Tucana III. The large velocity gradient of the stream implies that Tucana III is likely on a radial orbit. We successfully obtain metallicities for 4 members in the core and 12 members in the tails. We find that members close to the ends of the stream tend to be more metal-poor than members in the core, indicating a possible metallicity gradient between the center of the progenitor halo and its edge. The spread in metallicity suggests that the progenitor of the Tucana III stream is a dwarf galaxy rather than a star cluster. Furthermore, we find that with the precise photometry of the Dark Energy Survey data, there is a discernible color offset between metal-rich disk stars and metal-poor stream members. This metallicity-dependent color offers a more efficient method to recognize metal-poor targets and will increase the selection efficiency of stream members for future spectroscopic follow-up programs on stellar streams.

==> obstable.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[]
\centering
\caption{Observations}
\label{table:obs}
\begin{tabular}{l|c|c|c|c|l}
\hline \hline
\multirow{2}{*}{\textbf{Date}} & \multicolumn{3}{c|}{\textbf{Exp Time (s)}}                                     & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}seeing\\ ('')\end{tabular}}} & \multirow{2}{*}{\textbf{conditions}} \\ \cline{2-4}
                               & \begin{tabular}[c]{@{}c@{}}\code{AAT-Field-1}\\ 23h$\,$50m$\,$16.6s \\ $-$59$^\circ\,$36$'\,$00$''$\end{tabular} & \begin{tabular}[c]{@{}c@{}}\code{AAT-Field-2}\\ 00h$\,$02m$\,$55.4s \\ $-$59$^\circ\,$36$'\,$00$''$\end{tabular} & \begin{tabular}[c]{@{}c@{}}\code{AAT-Field-3}\\ 23h$\,$47m$\,$06.9s \\ $-$59$^\circ\,$36$'\,$00$''$\end{tabular} &                                                                         &                                      \\ \hline
2016 Jun 30                    & 3300                                                       &         &         & 1.9                                                                            & cloudy                               \\ \hline
2016 Jul 09                    & 9475                                                       & 750     &         & 2.3                                                                            & high humidity                        \\ \hline
2016 Jul 10                    & 5400                                                       & 7200    &         & 2.3                                                                            & cloudy                              \\ \hline
2016 Jul 12                    & 7800                                                       & 7200    &         & 3.0                                                                            & cloudy                               \\ \hline
2016 Jul 13                    &                                                            & 9000    &         & 3.2                                                                            & cloudy                                \\ \hline
2016 Jul 25                    & 7200                                                       & 9000    &         & 2.0                                                                            & clear                               \\ \hline
2016 Jul 26                    & 3200                                                       & 2460    &         & 2.5                                                                            & cloudy                              \\ \hline
2016 Jul 27                    & 2400                                                       & 700     &         & 4.0                                                                            & cloudy                               \\ \hline
2017 Aug 22                    &                                                            &         & 5400    & 1.9                                                                            & clear                               \\ \hline
\end{tabular}
\end{table*}

==> table_append_old.tex <==
\begin{deluxetable*}{c r r c c c c c c c}
\tabletypesize{\scriptsize}
\tablecaption{Potential members in the Tuc~III stream.
\label{tab:tuc3_spec_pot}
}
%\tablenum{2}
\tablehead{ID & $\alpha_{2000}$ & $\delta_{2000}$  & $g$ & $r$ & Cat & Inst & S/N & \multicolumn{1}{c}{$v$}  &$\sigma_{\mu}$\\ 
 & (deg) & (deg) & (mag) & (mag) &  &   &  & \multicolumn{1}{c}{(\kms)} & (mas/yr) }

\startdata
DES\,J233957.91$-$593718.3 & 354.99128 & -59.62174 & 19.392 & 18.950 & DR1 & AAT &  5.1 & -126.85 & 0.634\\
DES\,J234209.92$-$594724.9 & 355.54135 & -59.79024 & 19.806 & 19.398 & DR1 & AAT &  2.4 & -129.83 & 0.883\\
DES\,J234258.94$-$591925.4 & 355.74557 & -59.32372 & 19.784 & 19.363 & DR1 & AAT &  6.0 & -112.15 & 0.861\\
DES\,J234310.16$-$595556.6 & 355.79232 & -59.93240 & 20.956 & 20.758 & DR1 & AAT &  3.1 &  -82.66 & 2.672\\
DES\,J234311.08$-$590221.5 & 355.79615 & -59.03932 & 19.330 & 18.851 & DR1 & AAT &  2.2 &  -73.82 & 0.584\\
DES\,J234325.17$-$594435.1 & 355.85489 & -59.74308 & 18.763 & 18.320 & DR1 & AAT &  4.5 &  -82.15 & 0.397\\
DES\,J234354.41$-$600605.7 & 355.97671 & -60.10158 & 20.548 & 20.333 & DR1 & AAT &  1.7 & -108.10 & 1.853\\
DES\,J234446.62$-$601636.3 & 356.19427 & -60.27674 & 19.777 & 19.363 & DR1 & AAT &  5.6 & -113.56 & 0.860\\
DES\,J234502.83$-$594108.5 & 356.26180 & -59.68569 & 20.696 & 20.437 & DR1 & AAT &  2.1 &  -96.39 & 1.996\\
DES\,J234539.31$-$600534.8 & 356.41378 & -60.09300 & 20.413 & 20.165 & DR1 & AAT &  3.3 &  -85.55 & 1.617\\
DES\,J234653.40$-$600737.8 & 356.72251 & -60.12717 & 19.906 & 19.502 & DR1 & AAT &  5.3 & -114.54 & 0.959\\
DES\,J234703.67$-$592837.7 & 356.76528 & -59.47714 & 19.933 & 19.527 & DR1 & AAT &  4.7 & -135.28 & 0.979\\
DES\,J234722.75$-$601040.8 & 356.84479 & -60.17799 & 20.271 & 19.968 & DR1 & AAT &  2.0 & -100.87 & 1.382\\
DES\,J234754.05$-$593615.2 & 356.97523 & -59.60422 & 20.103 & 19.714 & DR1 & AAT &  4.2 & -117.72 & 1.137\\
DES\,J234801.37$-$591054.6 & 357.00572 & -59.18182 & 20.386 & 20.146 & DR1 & AAT &  3.1 & -117.09 & 1.587\\
DES\,J234822.42$-$600631.7 & 357.09343 & -60.10880 & 20.910 & 20.687 & DR1 & AAT &  6.5 & -103.71 & 2.516\\
DES\,J234854.73$-$593421.6 & 357.22804 & -59.57266 & 20.534 & 20.302 & DR1 & AAT &  1.9 & -132.98 & 1.809\\
DES\,J234907.03$-$595451.4 & 357.27929 & -59.91428 & 20.790 & 20.569 & DR1 & AAT &  3.7 &  -90.85 & 2.270\\
DES\,J234916.70$-$595028.3 & 357.31959 & -59.84118 & 20.457 & 20.231 & DR1 & AAT &  3.8 & -125.84 & 1.704\\
DES\,J234934.85$-$594127.9 & 357.39519 & -59.69107 & 20.718 & 20.501 & DR1 & AAT &  1.9 & -130.20 & 2.143\\
DES\,J234955.16$-$593738.0 & 357.47985 & -59.62722 & 20.374 & 20.128 & DR1 & AAT &  4.0 & -112.21 & 1.569\\
DES\,J235011.85$-$592433.7 & 357.54936 & -59.40936 & 20.308 & 20.025 & DR1 & AAT &  3.3 & -137.01 & 1.446\\
DES\,J235105.24$-$594437.3 & 357.77182 & -59.74369 & 20.372 & 20.098 & DR1 & AAT &  2.8 & -111.33 & 1.536\\
DES\,J235134.95$-$594124.6 & 357.89564 & -59.69016 & 19.846 & 19.411 & DR1 & AAT &  3.9 & -110.51 & 0.895\\
DES\,J235151.98$-$594056.9 & 357.96659 & -59.68247 & 19.806 & 19.377 & DR1 & AAT &  6.2 & -111.75 & 0.871\\
DES\,J235209.62$-$590450.5 & 358.04007 & -59.08070 & 19.844 & 19.411 & DR1 & AAT &  5.8 & -111.49 & 0.897\\
DES\,J235258.81$-$594111.3 & 358.24505 & -59.68646 & 20.553 & 20.337 & DR1 & AAT &  1.6 & -123.43 & 1.862\\
DES\,J235318.39$-$593243.8 & 358.32662 & -59.54549 & 20.422 & 20.179 & DR1 & IMACS &  4.5 & -100.10 & 1.638\\
DES\,J235328.33$-$593731.2 & 358.36804 & -59.62533 & 21.523 & 21.271 & DR1 & IMACS &  2.3 & -107.67 & 4.249\\
DES\,J235341.40$-$592600.9 & 358.42251 & -59.43358 & 19.796 & 19.329 & DR1 & AAT &  3.6 &  -93.32 & 0.843\\
DES\,J235400.65$-$593255.5 & 358.50273 & -59.54876 & 20.414 & 20.195 & DR1 & IMACS &  5.5 &  -99.64 & 1.660\\
DES\,J235408.52$-$594422.1 & 358.53551 & -59.73947 & 20.282 & 19.984 & DR1 & AAT &  2.8 &  -83.00 & 1.400\\
DES\,J235425.68$-$595943.3 & 358.60701 & -59.99537 & 20.313 & 20.002 & DR1 & AAT &  1.9 &  -93.49 & 1.426\\
DES\,J235425.87$-$594042.6 & 358.60780 & -59.67849 & 20.494 & 20.269 & DR1 & IMACS &  5.7 & -107.18 & 1.768\\
DES\,J235439.51$-$594118.7 & 358.66463 & -59.68854 & 19.997 & 19.611 & DR1 & AAT &  4.3 &  -83.00 & 1.045\\
DES\,J235544.46$-$591918.1 & 358.93527 & -59.32169 & 20.427 & 20.185 & DR1 & AAT &  4.3 & -120.70 & 1.640\\
DES\,J235549.61$-$592446.4 & 358.95673 & -59.41289 & 20.274 & 19.894 & DR1 & AAT &  3.1 & -135.94 & 1.278\\
DES\,J235615.37$-$595231.4 & 359.06405 & -59.87540 & 20.314 & 20.035 & DR1 & AAT &  2.3 &  -71.16 & 1.456\\
DES\,J235619.28$-$592219.0 & 359.08034 & -59.37195 & 20.788 & 20.560 & DR1 & AAT &  2.0 &  -93.64 & 2.260\\
DES\,J235634.89$-$593001.2 & 359.14537 & -59.50032 & 21.268 & 21.056 & DR1 & AAT &  2.6 & -108.97 & 3.489\\
DES\,J235712.70$-$600747.5 & 359.30291 & -60.12986 & 20.004 & 19.608 & DR1 & AAT &  3.1 & -116.45 & 1.046\\
DES\,J235901.96$-$592204.5 & 359.75815 & -59.36790 & 20.071 & 19.681 & DR1 & AAT &  2.1 &  -87.20 & 1.109\\
DES\,J000101.57$-$593029.7 &   0.25654 & -59.50824 & 19.631 & 19.184 & DR1 & AAT &  4.5 &  -96.29 & 0.751\\
DES\,J000105.45$-$592448.8 &   0.27272 & -59.41355 & 19.726 & 19.265 & DR1 & AAT &  4.3 & -100.99 & 0.800\\
DES\,J000133.88$-$595528.8 &   0.39116 & -59.92467 & 20.390 & 20.171 & DR1 & AAT &  2.2 & -106.77 & 1.619\\
DES\,J000336.20$-$595212.8 &   0.90082 & -59.87023 & 20.262 & 19.941 & DR1 & AAT &  1.8 & -100.49 & 1.360\\
DES\,J000400.30$-$593024.9 &   1.00126 & -59.50691 & 19.645 & 19.201 & DR1 & AAT &  4.5 &  -94.87 & 0.761\\
DES\,J000505.18$-$593122.1 &   1.27159 & -59.52280 & 20.825 & 20.620 & DR1 & AAT &  2.0 & -117.23 & 2.374\\
DES\,J000731.43$-$593438.7 &   1.88097 & -59.57741 & 20.819 & 20.592 & DR1 & AAT &  5.4 & -104.87 & 2.266\\
DES\,J000826.30$-$593212.2 &   2.10958 & -59.53672 & 19.218 & 18.742 & DR1 & AAT &  6.7 &  -93.81 & 0.539\\
DES\,J000841.53$-$591007.3 &   2.17302 & -59.16870 & 19.460 & 18.995 & DR1 & AAT &  2.7 &  -86.19 & 0.651\\
DES\,J000902.34$-$594247.1 &   2.25975 & -59.71310 & 19.828 & 19.409 & DR1 & AAT &  4.7 &  -71.10 & 0.890\\
\enddata
\tablecomments{
Stars that are observed with AAT or IMACS and have the measured RVs in the range of $-140~\kms < v < -70~\kms$, but the S/N of the spectra are too low to obtain robust velocity measurements, and therefore these stars are not included in the analysis. RVs should be used with caution. See details in Appendix~\ref{sec:moremember}.
}
\end{deluxetable*}

==> table_gaia.tex <==
\begin{deluxetable*}{c r r  c}
\tabletypesize{\scriptsize}
\tablecaption{Projected proper motion precision of the 29 spectroscopically confirmed members from AAT.
\label{tab:tuc3_gaia}
}
%\tablenum{2}
\tablehead{ID & $\alpha_{2000}$ & $\delta_{2000}$  & $\sigma_{\mu}$\\ 
 & (deg) & (deg) & (mas/yr) }

\startdata
DES\,J234327.66$-$593542.1 & 355.86526 & -59.59502 & 0.441 \\
DES\,J234350.83$-$593925.6 & 355.96177 & -59.65712 & 0.187 \\
DES\,J234434.87$-$594407.7 & 356.14531 & -59.73549 & 0.290 \\
DES\,J234521.78$-$593131.3 & 356.34076 & -59.52536 & 0.597 \\
DES\,J234531.06$-$593908.6 & 356.37941 & -59.65240 & 0.189 \\
DES\,J234642.46$-$601828.1 & 356.67692 & -60.30780 & 0.477 \\
DES\,J234642.83$-$593152.8 & 356.67844 & -59.53133 & 0.671 \\
DES\,J234654.06$-$594331.7 & 356.72524 & -59.72548 & 0.201 \\
DES\,J234702.14$-$594843.2 & 356.75890 & -59.81200 & 0.315 \\
DES\,J234719.86$-$595348.0 & 356.83277 & -59.89668 & 0.647 \\
DES\,J234727.52$-$591504.9 & 356.86466 & -59.25137 & 0.282 \\
DES\,J235248.09$-$602054.9 & 358.20036 & -60.34857 & 0.203 \\
DES\,J235349.12$-$593245.4 & 358.45467 & -59.54593 & 0.328 \\
DES\,J235532.68$-$593115.0 & 358.88616 & -59.52083 & 0.075 \\
DES\,J235549.92$-$593259.7 & 358.95799 & -59.54990 & 0.159 \\
DES\,J235620.76$-$593310.2 & 359.08651 & -59.55282 & 0.415 \\
DES\,J235650.50$-$593421.0 & 359.21042 & -59.57250 & 0.961 \\
DES\,J235707.46$-$593743.0 & 359.28110 & -59.62861 & 0.818 \\
DES\,J235726.04$-$593938.2 & 359.35851 & -59.66061 & 0.562 \\
DES\,J235730.25$-$592930.7 & 359.37602 & -59.49186 & 0.595 \\
DES\,J235738.50$-$593611.7 & 359.41040 & -59.60325 & 0.139 \\
DES\,J235745.46$-$593726.5 & 359.43941 & -59.62401 & 0.873 \\
DES\,J000234.74$-$593056.8 &   0.64473 & -59.51578 & 0.597 \\
DES\,J000347.26$-$593114.6 &   0.94693 & -59.52072 & 0.502 \\
DES\,J000427.21$-$593648.3 &   1.11336 & -59.61342 & 0.389 \\
DES\,J000529.05$-$600323.4 &   1.37102 & -60.05651 & 0.204 \\
DES\,J000548.69$-$593406.1 &   1.45288 & -59.56835 & 0.108 \\
DES\,J000639.63$-$591658.5 &   1.66513 & -59.28291 & 0.399 \\
DES\,J000727.58$-$593357.0 &   1.86493 & -59.56584 & 0.572 \\
\enddata
%\tablecomments{}
\end{deluxetable*}

==> table_old.tex <==
%\LongTables
%\begin{landscape}


\begin{deluxetable*}{c r r c c c c r r c c c c c c}
\tabletypesize{\scriptsize}
\tablecaption{Velocity and metallicity measurements of the observed stars.\tablenotemark{a}
\label{tab:tuc3_spec}
}
%\tablenum{2}

\tablehead{ID & dwarf & $\alpha_{2000}$ & $\delta_{2000}$  & $g$\tablenotemark{b} & $r$\tablenotemark{b} & Cat\tablenotemark{b} & Inst\tablenotemark{c} & S/N & \multicolumn{1}{c}{$v$} & ${\rm EW}$ & ${\rm [Fe/H]}$ & Mem\tablenotemark{d} & Prob\tablenotemark{e} &$\sigma_{\mu}$\tablenotemark{f} & Comment\\ 
 & (deg) & (deg) & (mag) & (mag) &  &   &  & \multicolumn{1}{c}{(\kms)} & (\AA) &  &  & & (mas/yr) &}


\startdata
 \multicolumn{15}{c}{ \ruleline{Tucana III Leading/West Tail} } \\
DES\,J234319.89$-$592540.8 & 355.83288 & $-$59.42799 & 18.194 & 17.719 & DR1 & AAT & 22.2 & $-72.93 \pm 0.98$ & $5.01 \pm 0.36$ & \noinfo &  0 & 0.00 & \noinfo &     \\
DES\,J234327.66$-$593542.1 & 355.86526 & $-$59.59502 & 18.931 & 18.465 & DR1 & AAT & 12.9 & $-116.19 \pm 1.79$ & $1.30 \pm 0.32$ & $-2.97 \pm 0.29$ &  1 & 1.00 & 0.441 &     \\
DES\,J234350.83$-$593925.6 & 355.96177 & $-$59.65712 & 17.678 & 17.151 & Y2Q & AAT & 33.8 & $-115.46 \pm 0.76$ & $1.83 \pm 0.30$ & $-2.83 \pm 0.18$ &  1 & 1.00 & 0.187 &   binary  \\
DES\,J234434.87$-$594407.7 & 356.14531 & $-$59.73549 & 18.339 & 17.835 & DR1 & AAT & 20.8 & $-115.27 \pm 1.23$ & $2.15 \pm 0.49$ & $-2.51 \pm 0.27$ &  1 & 0.99 & 0.290 &     \\
DES\,J234437.03$-$595405.6 & 356.15431 & $-$59.90157 & 17.005 & 16.391 & DR1 & AAT & 40.7 & $-75.88 \pm 0.77$ & $5.49 \pm 0.27$ & \noinfo &  0 & 0.00 & \noinfo &     \\
DES\,J234521.78$-$593131.3 & 356.34076 & $-$59.52536 & 19.340 & 18.883 & DR1 & AAT &  9.6 & $-116.09 \pm 2.43$ & $1.65 \pm 0.52$ & $-2.62 \pm 0.36$ &  1 & 0.99 & 0.597 &     \\
DES\,J234531.06$-$593908.6 & 356.37941 & $-$59.65240 & 17.672 & 17.127 & DR1 & AAT & 36.0 & $-110.38 \pm 0.84$ & $2.27 \pm 0.38$ & $-2.59 \pm 0.20$ &  1 & 0.98 & 0.189 &     \\
DES\,J234642.46$-$601828.1 & 356.67692 & $-$60.30780 & 19.046 & 18.576 & DR1 & AAT &  9.8 & $-114.02 \pm 3.39$ & $2.01 \pm 0.49$ & $-2.44 \pm 0.34$ &  1 & 0.98 & 0.477 &     \\
DES\,J234642.83$-$593152.8 & 356.67844 & $-$59.53133 & 19.487 & 19.038 & DR1 & AAT &  8.7 & $-114.70 \pm 3.08$ & $1.85 \pm 0.79$ & $-2.47 \pm 0.52$ &  1 & 0.97 & 0.671 &     \\
DES\,J234654.06$-$594331.7 & 356.72524 & $-$59.72548 & 17.240 & 17.395 & DR1 & AAT & 21.7 & $-109.61 \pm 1.61$ & \noinfo & \noinfo &  1 & 0.91 & 0.201 &  BHB  \\
DES\,J234702.14$-$594843.2 & 356.75890 & $-$59.81200 & 18.459 & 17.967 & DR1 & AAT & 17.7 & $-109.26 \pm 1.52$ & $1.99 \pm 0.59$ & $-2.58 \pm 0.34$ &  1 & 0.99 & 0.315 &     \\
DES\,J234719.86$-$595348.0 & 356.83277 & $-$59.89668 & 19.449 & 18.989 & DR1 & AAT &  8.9 & $-110.65 \pm 2.68$ & \noinfo & \noinfo &  1 & 0.92 & 0.647 &     \\
DES\,J234727.52$-$591504.9 & 356.86466 & $-$59.25137 & 18.296 & 17.789 & DR1 & AAT & 23.1 & $-111.07 \pm 0.99$ & $2.23 \pm 0.43$ & $-2.48 \pm 0.24$ &  1 & 1.00 & 0.282 &     \\
DES\,J234949.16$-$602020.5 & 357.45482 & $-$60.33902 & 18.137 & 17.596 & DR1 & AAT &  6.2 & $-113.59 \pm 3.12$ & \noinfo & \noinfo &  0 & 0.74 & \noinfo &     \\
DES\,J235158.27$-$591210.9 & 357.99278 & $-$59.20303 & 17.541 & 17.271 & Y2Q & AAT & 31.7 & $-88.46 \pm 0.84$ & $4.98 \pm 0.28$ & \noinfo &  0 & 0.00 & \noinfo &     \\
DES\,J235248.09$-$602054.9 & 358.20036 & $-$60.34857 & 17.265 & 17.404 & DR1 & AAT & 16.3 & $-105.58 \pm 2.57$ & \noinfo & \noinfo &  1 & 0.90 & 0.203 &   BHB  \\
DES\,J235349.12$-$593245.4 & 358.45467 & $-$59.54593 & 18.524 & 18.025 & DR1 & AAT & 17.1 & $-102.56 \pm 2.51$ & $2.41 \pm 0.46$ & $-2.34 \pm 0.25$ &  1 & 0.98 & 0.328 &     \\
DES\,J235349.12$-$593245.4 & 358.45467 & $-$59.54593 & 18.524 & 18.025 & DR1 & IMACS & 28.8 & $-103.61 \pm 1.04$ & $2.60 \pm 0.21$ & $-2.25 \pm 0.12$ &  1 & \noinfo & \noinfo &     \\
DES\,J235425.88$-$594103.3 & 358.60784 & $-$59.68424 & 20.288 & 20.008 & DR1 & IMACS &  6.8 & $-102.65 \pm 2.64$ & \noinfo & \noinfo &  1 & \noinfo & \noinfo &   subgiant  \\
DES\,J235435.00$-$593946.0 & 358.64582 & $-$59.66279 & 20.695 & 20.493 & DR1 & IMACS &  4.1 & $-100.63 \pm 3.24$ & \noinfo & \noinfo &  1 & \noinfo & \noinfo &  MSTO   \\
DES\,J235439.51$-$594118.7 & 358.66463 & $-$59.68854 & 19.997 & 19.611 & DR1 & IMACS &  9.7 & $-71.48 \pm 1.75$ & $1.87 \pm 0.29$ & \noinfo &  0 & \noinfo & \noinfo &     \\
 \multicolumn{15}{c}{ \ruleline{Tucana III Core\tablenotemark{g} } } \\
DES\,J235532.68$-$593115.0 & 358.88616 & $-$59.52083 & 16.090 & 15.344 & DR1 & AAT & 125.7 & $-102.89 \pm 0.51$ & $3.75 \pm 0.22$ & $-2.28 \pm 0.10$ &  1 & 0.99 & 0.075 &     \\
DES\,J235549.92$-$593259.7 & 358.95799 & $-$59.54990 & 17.400 & 16.815 & DR1 & AAT & 22.0 & $-101.94 \pm 1.40$ & $2.84 \pm 0.29$ & $-2.37 \pm 0.14$ &  1 & 1.00 & 0.159 &     \\
DES\,J235620.76$-$593310.2 & 359.08651 & $-$59.55282 & 18.857 & 18.374 & DR1 & AAT & 11.6 & $-101.83 \pm 2.19$ & $2.33 \pm 0.27$ & $-2.31 \pm 0.16$ &  1 & 0.99 & 0.415 &     \\
DES\,J235650.50$-$593421.0 & 359.21042 & $-$59.57250 & 19.950 & 19.496 & DR1 & AAT &  6.0 & $-102.12 \pm 4.99$ & \noinfo & \noinfo &  1 & 0.83 & 0.961 &     \\
DES\,J235707.46$-$593743.0 & 359.28110 & $-$59.62861 & 19.727 & 19.296 & DR1 & AAT &  5.7 & $-104.53 \pm 4.82$ & \noinfo & \noinfo &  1 & 0.81 & 0.818 &     \\
DES\,J235726.04$-$593938.2 & 359.35851 & $-$59.66061 & 19.265 & 18.800 & DR1 & AAT & 13.2 & $-101.89 \pm 2.64$ & \noinfo & \noinfo &  1 & 0.89 & 0.562 &     \\
DES\,J235730.25$-$592930.7 & 359.37602 & $-$59.49186 & 19.342 & 18.878 & DR1 & AAT &  8.1 & $-100.06 \pm 3.19$ & \noinfo & \noinfo &  1 & 0.88 & 0.595 &     \\
DES\,J235738.50$-$593611.7 & 359.41040 & $-$59.60325 & 17.173 & 16.569 & DR1 & AAT & 45.9 & $-99.58 \pm 0.71$ & $2.66 \pm 0.25$ & $-2.50 \pm 0.13$ &  1 & 1.00 & 0.139 &     \\
DES\,J235745.46$-$593726.5 & 359.43941 & $-$59.62401 & 19.806 & 19.379 & DR1 & AAT &  8.2 & $-100.01 \pm 3.29$ & \noinfo & \noinfo &  1 & 0.88 & 0.873 &     \\
 \multicolumn{15}{c}{ \ruleline{Tucana III Trailing/East Tail} } \\
DES\,J235853.63$-$595952.2 & 359.72345 & $-$59.99784 & 18.956 & 18.467 & DR1 & AAT & 10.3 & $-121.84 \pm 2.14$ & $3.87 \pm 0.63$ & \noinfo &  0 & 0.00 & \noinfo &     \\
DES\,J235855.20$-$591242.4 & 359.73001 & $-$59.21177 & 18.701 & 18.219 & DR1 & AAT &  9.8 & $-78.54 \pm 2.86$ & $2.16 \pm 0.29$ & \noinfo &  0 & 0.00 & \noinfo &     \\
DES\,J235855.20$-$591242.4 & 359.73001 & $-$59.21177 & 18.701 & 18.219 & DR1 & IMACS &  6.6 & $-74.02 \pm 1.52$ & \noinfo & \noinfo &  0 & \noinfo & \noinfo &     \\
DES\,J000104.89$-$594814.4 &   0.27039 & $-$59.80400 & 18.833 & 18.394 & DR1 & AAT &  8.0 & $-85.13 \pm 4.37$ & $2.19 \pm 0.60$ & \noinfo &  0 & 0.49 & \noinfo &     \\
DES\,J000234.74$-$593056.8 &   0.64473 & $-$59.51578 & 19.341 & 18.881 & DR1 & AAT &  5.7 & $-92.26 \pm 4.46$ & \noinfo & \noinfo &  1 & 0.78 & 0.597 &     \\
DES\,J000344.78$-$600048.2 &   0.93656 & $-$60.01339 & 19.109 & 18.670 & DR1 & AAT &  7.8 & $-129.28 \pm 3.42$ & \noinfo & \noinfo &  0 & 0.00 & \noinfo &     \\
DES\,J000347.26$-$593114.6 &   0.94693 & $-$59.52072 & 19.104 & 18.646 & DR1 & AAT &  7.1 & $-93.82 \pm 3.38$ & \noinfo & \noinfo &  1 & 0.86 & 0.502 &     \\
DES\,J000427.21$-$593648.3 &   1.11336 & $-$59.61342 & 18.771 & 18.283 & DR1 & AAT & 10.7 & $-94.58 \pm 2.58$ & \noinfo & \noinfo &  1 & 0.87 & 0.389 &     \\
DES\,J000529.05$-$600323.4 &   1.37102 & $-$60.05651 & 17.543 & 17.318 & DR1 & AAT & 21.6 & $-91.05 \pm 2.97$ & \noinfo & \noinfo &  1 & 0.85 & 0.204 &   RHB  \\
DES\,J000548.69$-$593406.1 &   1.45288 & $-$59.56835 & 16.770 & 16.123 & Y2Q & AAT & 40.4 & $-92.01 \pm 0.70$ & $2.34 \pm 0.35$ & $-2.75 \pm 0.18$ &  1 & 1.00 & 0.108 &     \\
DES\,J000639.63$-$591658.5 &   1.66513 & $-$59.28291 & 18.813 & 18.316 & DR1 & AAT &  9.8 & $-92.11 \pm 2.30$ & $2.09 \pm 0.27$ & $-2.46 \pm 0.16$ &  1 & 0.99 & 0.399 &     \\
DES\,J000727.58$-$593357.0 &   1.86493 & $-$59.56584 & 19.321 & 18.865 & Y2Q & AAT &  7.3 & $-92.58 \pm 3.35$ & \noinfo & \noinfo &  1 & 0.82 & 0.572 &     \\
DES\,J000758.93$-$594729.2 &   1.99552 & $-$59.79145 & 18.530 & 18.038 & DR1 & AAT & 11.7 & $-99.87 \pm 2.08$ & $5.83 \pm 0.58$ & \noinfo &  0 & 0.00 & \noinfo &     \\
\enddata
\tablecomments{\\
(a) Only stars with $ -140 < \vhel < -70 ~\kms$ are presented here. The remaining measurements are available in the online version in machine readable format.\\ 
(b) Quoted magnitudes represent the dereddened PSF magnitude in either DR1 or Y2Q catalog.\\
(c) Telescopes and instruments used for obtaining the spectra of the targets. AAT stands for AAT/2df+AAOmega; IMACS stands for Magellan/IMACS. \\
(d) The membership of Tuc~III stream stars through a subjective membership identification (see details in \S\ref{sec:membership}). Mem = 1 are members; Mem = 0 are non-members.\\
(e) The membership probability of Tuc~III stream stars through an objective mixture model. Measurements from the AAT observations are used for modeling. See details in \S\ref{sec:mixture}). \\
(f) The projected proper motion precision from \gaia DR2 on the member stars of Tuc~III stream (see details in Appendix~\ref{sec:pmprecision}).\\
(g) These 9 Tuc~III core members are also observed by ~\citet{tuc3}.
}
%\tablenotetext{a}{Quoted magnitudes represent the weighted-average dereddened PSF magnitude derived from the DES images using SExtractor \citep{dw15b}.}(a) Only stars with $ -140 < \vhel < -70 ~\kms$ are presented here. The remaining measurements are available in the online version in machine readable format.\\ (b) Quoted magnitudes represent the dereddened PSF magnitude derived from either DR1 or Y2Q catalog.
\end{deluxetable*}

%\end{landscape}
